AutoTVG: A New Vision-language Pre-training Paradigm for Temporal Video Grounding

Temporal Video Grounding (TVG) aims to localize a moment from an untrimmed video given the language description. Since the annotation of TVG is labor-intensive, TVG under limited supervision has accepted attention in recent years. The great success of vision-language pre-training guides TVG to follow the traditional "pre-training + fine-tuning" paradigm, however, the pre-training process would suffer from a lack of temporal modeling and fine-grained alignment due to the difference of data nature between pre-train and test. Besides, the large gap between pretext and downstream tasks makes zero-shot testing impossible for the pre-trained model. To avoid the drawbacks of the traditional paradigm, we propose AutoTVG, a new vision-language pre-training paradigm for TVG that enables the model to learn semantic alignment and boundary regression from automatically annotated untrimmed videos. To be specific, AutoTVG consists of a novel Captioned Moment Generation (CMG) module to generate captioned moments from untrimmed videos, and TVGNet with a regression head to predict localization results. Experimental results on Charades-STA and ActivityNet Captions show that, regarding zero-shot temporal video grounding, AutoTVG achieves highly competitive performance with in-distribution methods under out-of-distribution testing, and is superior to existing pre-training frameworks with much less training data.

==> anet_exp.tex <==
\section{Experimental results on ActivityNet Captions}
\label{sec:anet_exp}


For a fair comparison with existing methods~\cite{nam2021zero} and ~\cite{wang2022prompt}, we conduct experiments on ActivityNet Captions dataset with C3D feature pre-trained on Sports-1M dataset~\cite{krishna2017dense}, see~\cref{tab:c3d_anet}. In detail, we follow~\cite{krishna2017dense} to extract C3D features, firstly we decode HowTo100M videos at 2 fps, then extract a clip feature at every 8 frames and concatenate all clip features as a video feature (shape=$[N, 4096]$, $N$ is the number of clips). Finally, we apply PCA~\cite{abdi2010principal} to video features to decrease feature dimension from 4096 to 500. 
From ~\cref{tab:c3d_anet}, we can see ZeusTVG surpasses other counterparts with the same feature pre-training and testing.


\begin{table}
    \centering
    \begin{tabularx}{\linewidth}{cc*2{c}}
    \toprule
    \textbf{Method} & \textbf{Feature} & \textbf{R@0.3} & \textbf{R@0.5} \\
    \midrule[.1pt]
    \multicolumn{4}{c}{\textit{Fully-supervised}}\\
    %  ExCL~\cite{ghosh2019excl} (v2) & I3D & 62.30 & 42.70 & 24.10 \\
    %  VSLNet~\cite{zhang2020span} (v2) & I3D & 63.16 & 43.22 & 26.16 \\
    %  CCA~\cite{wu2022learning} (v2) & I3D & 61.99 & 46.58 & 29.37 \\
     MLVI~\cite{xu2019multilevel} & C3D & 45.30 & 27.70  \\
     TripNet~\cite{hahn2019tripping} & C3D & 48.42 & 32.19  \\
     ABLR~\cite{yuan2019find} & C3D & 55.67 & 36.79  \\
     LGI~\cite{mun2020local} & C3D & 58.52 & 41.51  \\
     TMLGA~\cite{rodriguez2020proposal} & I3D & 51.28 & 33.04  \\
     CBP~\cite{zhou2022thinking} & I3D & 54.30 & 35.76  \\
     BPNet~\cite{xiao2021boundary} & I3D & 58.98 & 42.07  \\
    \midrule[.1pt]
    \multicolumn{4}{c}{\textit{Weakly-supervised}}\\
     WSLLN~\cite{gao2019wslln} & C3D & 42.80 & 22.70  \\
     SCN~\cite{lin2020weakly} & C3D & 47.23 & 29.22  \\
     LCNet~\cite{yang2021local}& C3D  & 48.49 & 26.33 \\
     MARN~\cite{song2020weakly}& C3D  & 47.01 & 29.95  \\
     CTF~\cite{2020Look} & C3D  & 44.30 & 23.60 \\
    \midrule[.1pt]
    \multicolumn{4}{c}{\textit{Zero-shot}}\\
     DSCNet~\cite{liu2022unsupervised} & C3D & 47.29 & 28.16 \\
     \rowcolor{gray!20}
     PSVL~\cite{nam2021zero} & C3D & 44.74 &  30.08  \\
     \rowcolor{gray!20}
     PZVMR~\cite{wang2022prompt} & C3D & 45.73 & 31.26  \\
     \rowcolor{gray!20}
     PZVMR w/o $L_o$ ~\cite{wang2022prompt} & C3D & 43.54 & 29.35  \\
     ZeusTVG & CLIP & 36.16 & 15.60  \\
     \textbf{ZeusTVG} & \textbf{I3D}  & \textbf{39.31} & \textbf{21.31}  \\
     \textbf{ZeusTVG} &  C3D  &   &   \\
    \bottomrule
    \end{tabularx}
    \caption{Evaluation results on ActivityNet Captions. ZeusTVG shows superior performance in zero-shot setting. Methods in gray background conduct pseudo labeling and fine-tuning using ActivityNet Captions.}
    \label{tab:c3d_anet}
\end{table}

==> finetune.tex <==
\section{Fine-tuning Results on Downstream Datasets}
\label{sec:finetune}

To compare AutoTVG with the traditional ''pre-training + fine-tuning'' method, we also conduct experiments about fine-tuning downstream datasets on pre-trained TVGNet.

\begin{table}[]
    \centering
    \begin{tabular}{ccccc}
    \toprule
    Pre-train     &  Fix Text & \textbf{R@0.5} & \textbf{R@0.7} & \textbf{mIoU} \\  
    \midrule
    \checkmark   &  \checkmark   &  30.46   &  17.18  &  29.23   \\
    \checkmark   &  -   &  30.46   &   17.18   &   29.23  \\
    \checkmark   &  - CLIP & 21.64  &  6.80  &  25.47   \\
    \checkmark   &  \checkmark CLIP & 21.64  &  6.80  &  25.47   \\
    
    -    &  \checkmark &   41.40   &  18.74    &   39.72  \\
    -    &  -          &   45.51   &  22.26    &   41.22  \\
    -    &   \checkmark CLIP  &     &       &          \\
    
    \bottomrule
    \end{tabular}
    \vspace{1mm}
    \caption{Effectiveness of pre-training.}
    \label{tab:finetune}
\end{table}

==> locvtp.tex <==
\section{Comparison with other video temporal localization methods}
\label{sec:locvtp}

==> tables/grounding.tex <==

\begin{table}[]
\label{grounding}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|l|}{\multirow{}{}{Methods}} & \multicolumn{1}{l|}{\multirow{}{}{Mode}} & \multicolumn{3}{l|}{Charades-STA}                                                          & \multicolumn{4}{l|}{ActivityNet Captions}                                                                                 \\ \cline{3-9} 
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{l|}{}                      & \multicolumn{1}{l|}{R@1}     & \multicolumn{1}{l|}{R@1}     & \multicolumn{1}{l|}{R@1}     & \multicolumn{1}{l|}{R@1}     & \multicolumn{1}{l|}{R@1}     & \multicolumn{1}{l|}{R@5}     & \multicolumn{1}{l|}{R@5}     \\ \cline{3-9} 
\multicolumn{1}{|l|}{}                         & \multicolumn{1}{l|}{}                      & \multicolumn{1}{l|}{IoU=0.3} & \multicolumn{1}{l|}{IoU=0.5} & \multicolumn{1}{l|}{IoU=0.7} & \multicolumn{1}{l|}{IoU=0.3} & \multicolumn{1}{l|}{IoU=0.5} & \multicolumn{1}{l|}{IoU=0.3} & \multicolumn{1}{l|}{IoU=0.5} \\ \hline
Rondom                                         & FS                                         & 20.12                        & 8.51                         & 3.03                         & 18.64                        & 7.73                         & 52.78                        & 29.49                        \\
VSA-RNN                                        & FS                                         & 10.5                         & 4.32                         & 48.43                        & 70.84                        & 55.52                        &                              &                              \\
VSA-STV                                        & FS                                         & 16.91                        & 5.81                         & 53.89                        & 71.05                        & 56.62                        &                              &                              \\
CTRL                                           & FS                                         & 23.62                        & 8.89                         & 58.92                        &                              &                              &                              &                              \\
TGN                                            & FS                                         & 43.81                        & 27.93                        & 54.56                        &                              &                              &                              &                              \\
EFRC                                           & FS                                         & 53                           & 33.8                         & 15                           &                              &                              &                              &                              \\
2D-TAN                                         & FS                                         & 39.81                        & 23.25                        & 79.33                        & 85.53                        & 77.13                        &                              &                              \\
DRN                                            & FS                                         & 45.4                         & 26.4                         & 88.01                        &                              &                              &                              &                              \\\hline
TGA                                            & WS                                         & 32.14                        & 19.94                        & 8.84                         &                              &                              &                              &                              \\
SCN                                            & WS                                         & 42.96                        & 23.58                        & 9.97                         & 47.23                        & 29.22                        & 71.45                        & 55.69                        \\
CTF                                            & WS                                         & 39.8                         & 27.3                         & 12.9                         &                              &                              &                              &                              \\
MARN                                           & WS                                         & 48.55                        & 31.94                        & 14.18                        & 47.01                        & 29.95                        & 72.02                        & 57.49                        \\
VGN                                            & WS                                         & 32.21                        & 15.68                        & 73.5                         & 77.36                        & 61.29                        &                              &                          \\\hline 
PSVL & Zero-shot & 46.47 & 31.29 & 14.17 & 44.74 & 30.08 & &  \\\hline
\end{tabular}
\end{table}

==> tables/recognition.tex <==

\begin{table}[]
    \label{recognition}
    \centering
    \begin{tabular}{c|c|c|c|c|c}
    \hline
        Video Dataset& Method & Pretrain Dataset & Acc@1 & Acc@5 & AVG\\
    \hline
       Kinetics-400  &  & WebVid &  &   &  \\
                    & ActionCLIP &  CLIP  &  ~55  &   &  \\ 
    \hline
       Kinetics-700 & CLIP zero-shot  & CLIP(ViT-B-16)  &     &     &  52.4  \\
                    & CLIP zero-shot  & CLIP(ViT-B-32)  &     &     &  47.8  \\
                    & CLIP zero-shot  & CLIP(ViT-L-14)  &     &     &  60.3  \\
                    & CLIP linear probe(not zero-shot)  &  CLIP  &   &    &   66.1 \\
    \hline
       UCF-101 &   ActionCLIP  & Kinetics-400  &  ~70 &   & \\
                & & Kinetics-400/WebVid &   &   & \\
    \hline
       HMDB-51 &  ActionCLIP  & Kinetics-400  &   ~50  &  &    \\
                &   & Kinetics-400/WebVid & &   &  \\
    \hline
    \end{tabular}
    \caption{Zero-shot Video Recognition}

\end{table}



==> tables/retrieval.tex <==


\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c}
    \hline
        Video Dataset& Method & Pretrain Dataset & R@1 & R@5 & R@10 & MedR \\
    \hline
        MSR-VTT & Frozen-in-time & ImageNet/CC3M/WebVid &  18.7 & 39.5 & 51.6 & 10.0     \\
        1K-A MSR-VTT  & TimeSFormer  & WebVid &  13.0 & & 40.2 & 18.0 \\
                        & Frozen-in-time & WebVid & 14.6 & & 42.7 & 16.0 \\
    
    \hline
      
    \end{tabular}
    \caption{Zero-shot Video Retrieval}
    \label{retrieval}
\end{table}

